Riemannian Diffusion Models

Diffusion models are recent state-of-the-art methods for image generation and likelihood estimation. In this work, we generalize continuous-time diffusion models to arbitrary Riemannian manifolds and derive a variational framework for likelihood estimation. Computationally, we propose new methods for computing the Riemannian divergence which is needed in the likelihood estimation. Moreover, in generalizing the Euclidean case, we prove that maximizing this variational lower-bound is equivalent to Riemannian score matching. Empirically, we demonstrate the expressive power of Riemannian diffusion models on a wide spectrum of smooth manifolds, such as spheres, tori, hyperboloids, and orthogonal groups. Our proposed method achieves new state-of-the-art likelihoods on all benchmarks.

==> notes.tex <==

Some references (google drive for some books \url{https://drive.google.com/drive/folders/1oR3Ih7azSZ8Ip_AEF7opyscbD46Jhu5Q?usp=sharing})
\begin{enumerate}
    \item ch8 of \citet{chirikjian2009stochastic} is related to SDE on manifold. 
    \item main variational framework \citet{huang2021variational}
    \item example 8.5.8 of \citet{oksendal2003stochastic} shows how to project SDE onto the unit sphere to obtain a new process
    \item Riemannian CNF \citep{mathieu2020riemannian}
    \item \label{FKM}Feynman-Kac formula for PDE on manifold \url{https://math.uni.lu/thalmaier/SDE_PDE/SDE_PDE.pdf} (Proposition 3.1, maybe try to find a better ref)
    \item Girsanov on Manifold \citep[p263]{elworthy1982stochastic}
    \item Convert multi-D stratonovic to it\^o: \label{str2ito} \url{https://books.google.nl/books?id=_WfwCAAAQBAJ&pg=PA137&lpg=PA137#v=onepage&q&f=false}
\end{enumerate}


TODOs:
\begin{enumerate}
    \item how to design SDE that will stay on manifold (see section 8.2 \citet{chirikjian2009stochastic})
    \item Solving FP for simple BM-like diffusion on simple manifolds 
    \begin{enumerate}
        \item circles and tori are done. \url{https://colab.research.google.com/drive/12RMp4PFr4phsic8A3VVZLdxn2ywSjve2?usp=sharing}
        \item How to solve the heat equation (on simple manifolds, such as circles, spheres and tori). This is to get a formula to sample from the transitional distribution corresponding to the inference process. 
    \end{enumerate}
    \item adapt \citet{huang2021variational} to derive a lower bound on marginal likelihood of diffusion model on manifold (cf. \citet{chirikjian2009stochastic} eq 8.2 for a manifold version of Fokker Planck)
    \begin{enumerate}
        \item sanity check of the feynman-kac formula on
        regrouping of terms on stratanovich sde on patch
        \item applying jensen inequality + girsanov theorem to get a lower bound
        \item (test manifold Fokker Planck + Feynman Kac (toy problem) by estimating p(x) directly using monte carlo (assigned to Milad?))
        \item proof that the divergence term is chart independent (from \href{https://arxiv.org/abs/2108.08052} {moserflow paper})+ are the other terms also chart independent! 
    \end{enumerate}
    \item Quickly test the idea on data lying on a circle (or torus). In this case the Riemannian metric will just be a constant. 
    
\end{enumerate}

Questions:
\begin{enumerate}
    \item work with which formulation of stochastic integral? Ito or Stratonovich?
    \item Intrinsic or extrinsic coordinate? 
\end{enumerate}

Some data that we can consider modeling
\begin{enumerate}
    \item sphere: Earth science, climate data, e.g. earthquake intensity / frequency. See \citet{mardia2009directional}
    \item learned manifold via an autoencoder (high dim)
    \item unitary Lie groups like U(1), SU(2), etc: standard model of particle physics (also see Woit et al 17')
\end{enumerate}


==> sanity.tex <==
\paragraph{Sanity check}
In order to do a simple sanity check, we check whether when $\gvol = \igvol = 1$, the formula reduces to this paper appendix D of~\citet{huang2021variational}.
We have:
\begin{align}
&b_i = 
        -(\tilde{V_0})_{i}
        +
        \frac{1}{2} \igvol
        \bigg(
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\gvol \sigma^{j,k} \big)
        +
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \frac{\partial}{\partial \tilde{x}_j} 
            \big(
                \sigma^{j,k}  \gvol \sigma^{i,k} 
            \big) 
        \bigg), \gvol = 1 \Rightarrow \\
&b_i = 
        -(\tilde{V_0})_{i}
        +
        \frac{1}{2}
        \bigg(
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big( \sigma^{j,k} \big)
        +
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \frac{\partial}{\partial \tilde{x}_j} 
            \big(
                \tilde{V_0}_{j,k}   \sigma^{i,k} 
            \big) 
        \bigg)
\end{align}
From reverse product rule we know that
\begin{align}
\sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big( \sigma^{j,k} \big) =
\frac{\partial}{\partial \tilde{x}_{j}} \big( \sigma^{i,k} \sigma^{j,k} \big) - \sigma^{j,k}  \frac{\partial}{\partial \tilde{x}_{j}}  \big( \sigma^{i,k} \big)
\end{align}


Plugging this in we have:
\begin{align}
&b_i = 
        -(\tilde{V_0})_{i}
        +
        \frac{1}{2}
        \bigg(
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \bigg(
        \frac{\partial}{\partial \tilde{x}_{j}} \big( \sigma^{i,k} \sigma^{j,k} \big) - \sigma^{j,k}  \frac{\partial}{\partial \tilde{x}_{j}}  \big( \sigma^{i,k} \big)
        \bigg)
        +
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \frac{\partial}{\partial \tilde{x}_j} 
            \big(
                \sigma^{j,k}   \sigma^{i,k} 
            \big) 
        \bigg)
\\&=
 -(\tilde{V_0})_{i}
        -
        \frac{1}{2}
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \sigma^{j,k}  \frac{\partial}{\partial \tilde{x}_{j}}  \big( \sigma^{i,k} \big)
        +
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \frac{\partial}{\partial \tilde{x}_j} 
            \big(
                \sigma^{j,k}   \sigma^{i,k} 
            \big) 
\\&=
-\mu^{i} + 
\sum_{j=1}^{d} 
        \sum_{k=1}^{w}
        \frac{\partial}{\partial \tilde{x}_j} 
            \big(
                \sigma^{j,k}   \sigma^{i,k} 
            \big) 
\end{align}
As we can see $b_i$ term is the same with the paper. Also, the $\sigma$ terms are equivalent. Therefore, the diffusion part is the same. Now, let us verify also the expectation part is the same.
\begin{align}
&p(x, t)=\mathbb{E}\left[\exp \left(\int_{0}^{t} V\left(X_{s}\right) \ddd s\right) p_0\left(X_{t}\right)\right]
=
\mathbb{E}\left[\exp 
\left( \int_{0}^{t} V\left(X_{s}\right) \ddd s \right)
p_0\left(X_{t}\right)
\right]\\
\end{align}
\begin{align}
&V =
\igvol  \Bigg( -\diverge (\gvol \tilde{V_0}) +
\frac{1}{2} 
\sum_{i=1}^{d}
\sum_{j=1}^{d} 
\sum_{k=1}^{w}
    \frac{\partial}{\partial \tilde{x}_i} 
        \Big(
            \sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\gvol \sigma^{j,k} \big)
        \Big)
\Bigg) \xrightarrow{\gvol = 1} \\&
=
-\diverge (\tilde{V_0}) +
\frac{1}{2} 
\sum_{i=1}^{d}
\sum_{j=1}^{d} 
\sum_{k=1}^{w}
    \frac{\partial}{\partial \tilde{x}_i} 
        \Big(
            \sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{j,k} \big)
        \Big)
\end{align}
Plugging this in we have:
\begin{align}
&p(x, t)=\mathbb{E}\left[\exp \left(\int_{0}^{t} V\left(X_{s}\right) \ddd s\right) p_0\left(X_{t}\right)\right]
\\&= 
\mathbb{E}\left[\exp 
\left( 
    \int_{0}^{t} 
        -\diverge (\tilde{V_0}) +
        \frac{1}{2} 
        \sum_{i=1}^{d}
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
            \frac{\partial}{\partial \tilde{x}_i} 
                \Big(
                    \sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{j,k} \big)
                \Big)
    \ddd s 
\right)
p_0\left(X_{t}\right)
\right]\\
\end{align}
From reverse product rule we have that:
\begin{align}
\sigma^{i,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{j,k} \big)
= 
\frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{i,k}  \sigma^{j,k} \big)
-
\sigma^{j,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{i,k} \big)
\end{align}
Therefore, we can write that:
\begin{align}
&p(x, t)= 
\mathbb{E}\left[\exp 
\left( 
    \int_{0}^{t} 
        -\diverge (\tilde{V_0}) +
        \frac{1}{2} 
        \sum_{i=1}^{d}
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
            \frac{\partial}{\partial \tilde{x}_i} 
                \Big(
                    \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{i,k}  \sigma^{j,k} \big)
                    -
                    \sigma^{j,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{i,k} \big)
                \Big)
    \ddd s 
\right)
p_0\left(X_{t}\right)
\right]
\\&=
\mathbb{E}
\left[\exp 
\left( 
    \int_{0}^{t} 
        -\diverge (\tilde{V_0})
        -
        \frac{1}{2} 
        \sum_{i=1}^{d}
        \frac{\partial}{\partial \tilde{x}_i}
        \Big(
            \sum_{j=1}^{d} 
            \sum_{k=1}^{w}
                \sigma^{j,k}  \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{i,k} \big)
        \Big)
        +
        \frac{1}{2} 
        \sum_{i=1}^{d}
        \sum_{j=1}^{d} 
        \sum_{k=1}^{w}
            \frac{\partial}{\partial \tilde{x}_i} 
                \Big(
                    \frac{\partial}{\partial \tilde{x}_{j}} \big(\sigma^{i,k}  \sigma^{j,k} \big)
                \Big)
    \ddd s 
\right)
p_0\left(X_{t}\right)
\right]
\\&
=
\mathbb{E}
\left[\exp 
\left( 
    \int_{0}^{t} 
        -\diverge (\mu)
        +
        \sum_{i=1,j=1}^{d}
        \frac{1}{2} 
        \frac{\partial^2}{\partial \tilde{x}_i \partial \tilde{x}_{j}} 
        \big(\sigma^{i,k}  \sigma^{j,k} \big)
    \ddd s 
\right)
p_0\left(X_{t}\right)
\right]
\end{align}
As we can see this is the same as \citet{huang2021variational}.
